Hardware, Algorithms, and Applications of the Neuromorphic Vision Sensor: a Review

Neuromorphic, or event, cameras represent a transformation in the classical approach to visual sensing encodes detected instantaneous per-pixel illumination changes into an asynchronous stream of event packets. Their novelty compared to standard cameras lies in the transition from capturing full picture frames at fixed time intervals to a sparse data format which, with its distinctive qualities, offers potential improvements in various applications. However, these advantages come at the cost of reinventing algorithmic procedures or adapting them to effectively process the new data format. In this survey, we systematically examine neuromorphic vision along three main dimensions. First, we highlight the technological evolution and distinctive hardware features of neuromorphic cameras from their inception to recent models. Second, we review image processing algorithms developed explicitly for event-based data, covering key works on feature detection, tracking, and optical flow -which form the basis for analyzing image elements and transformations -as well as depth and pose estimation or object recognition, which interpret more complex scene structures and components. These techniques, drawn from classical computer vision and modern data-driven approaches, are examined to illustrate the breadth of applications for event-based cameras. Third, we present practical application case studies demonstrating how event cameras have been successfully used across various industries and scenarios. Finally, we analyze the challenges limiting widespread adoption, identify significant research gaps compared to standard imaging techniques, and outline promising future directions and opportunities that neuromorphic vision offers.

==> sections/5-slam.old.tex <==
\subsection{Camera Localization and Mapping}
\label{sec:poses}

Estimating a camera's 6-DoF pose is a fundamental problem of vision applications as it allows for the further development of autonomous systems, empowering robots with the capability of gaining situational awareness in entirely new environments~\cite{bavle2023slam}. 
When constructing a map of an unknown environment while simultaneously continuously estimating the camera's motion, we refer to the Simultaneous Localization and Mapping (SLAM) problem. The SLAM system could be considered a VO system with a mapping component that helps to maintain global consistency over time through loop closures~\cite{taketomi2017visual,Tsintotas2022}. 

In general, many sensors, from LIDAR to IMU, RADAR, Radio-Frequency, or a combination of these~\cite{kabiri2024graph}, have been employed with various degrees of success to perform SLAM. Using event cameras naturally brings the research in this field closer to the visual SLAM. Hence, we refer to the works in this area simply as SLAM. Another term linked with SLAM is visual odometry (VO). VO refers solely to estimating the position and orientation of a camera in real-time, based on the analysis of consecutive images captured by the camera, without caring for consistency on a global level. Hence, we can .


SLAM using event cameras is challenging due to the fundamental differences between events and images, which render conventional methods ineffective. Therefore, new SLAM techniques focus on preserving the low-latency nature of data. Hence, each incoming event may update the system's state asynchronously to exploit event camera properties in challenging scenarios. To this aim, Bayesian filters are popular in event-based SLAM because they are naturally suited for incrementally updating a system's state based on single observations. Therefore, many examples of this approach are found in the literature~\cite{Weikersdorfer2012, Weikersdorfer2013, Weikersdorfer2014, Kim2014, Censi2014, Gallego2018a}.

Event-based SLAM typically produces semi-dense maps that primarily consist of scene edges, which must be estimated along with the camera's motion since event cameras only measure temporal changes, not intensity gradients. The most general event-based SLAM problem, which involves a 6-DOF motion and natural 3D scenes, is a challenging problem addressed step-by-step in increasingly complex scenarios. For example,~\citet{Gallego2017}  focus on estimating the angular velocity with the contrast maximization approach robustly and accurately, which traditionally monocular cameras strive to perform. \citet{Reinbacher2017} perform panoramic reconstructions to track the global orientation of the camera. EVO~\cite{Rebecq2017} is a more complex method that tracks the full camera motion's degrees of freedom by aligning detected edges with an online reconstructed 3D semi-dense map only using event measurements.

Additional sensors may also be combined with NCs to reduce the complexity of the problem. For example,~\citet{Zhu2017} fuse inertial measurements with Extended Kalman Filters to estimate ego-motion at high frame rates. Ultimate SLAM~\cite{Vidal2018} exploits the IMU to track simple features extracted from event frame representations even in low light. Furthermore, multiple event cameras calibrated and time-synchronized in a stereo setup have also been tested with success~\cite{Zhou2021, Chen2022, Liu2023}. Finally, DEVO \cite{Zuo2022} is a recent method combining time surfaces with depth maps from RGB-D cameras to estimate the motion by 3D-2D edge alignment.



On the other hand, mapping allows for maintaining such consistency over time when places are visited multiple times and creates a loop closure. Several techniques can be used for mapping, jointly with establishing the camera motion between frames. For example, after confirming the distance to points or the 3D structure of the scene, a map can be created by integrating measurements over time in a Signed Distance Field (SDF) representation useful for planning or a sparser 3D point cloud, from which discarding outliers and culling superfluous 3D points reduce even further the memory footprint for efficient localization.

Traditionally, multi-view reconstruction involves identifying and matching corresponding points in multiple images and using these points to compute the position and orientation of each camera relative to the scene. Once the camera positions are known, the 3D coordinates,~\ie the depth is the remaining unknown parameter of points in the scene, can be estimated using techniques such as triangulation. The resulting 3D point cloud can generate a 3D mesh or surface representation of the object or scene. 

Monocular depth estimation is a challenging task that has garnered significant research attention in recent years due to its potential applications to autonomous robot navigation. Monocular depth estimation relies on a single camera compared to traditional stereo vision techniques, which use multiple synchronized cameras to estimate depth. Therefore, it requires innovative approaches to overcome the inherent lack of depth information. These methods can reconstruct a semi-dense 3D map in correspondence with edges by recovering the camera motion simultaneously. Therefore, this problem, albeit more challenging, is of greater interest when dealing with SLAM. 
Recent research has demonstrated successful monocular depth estimation with event cameras. These approaches integrate information from events captured over time by a moving camera. In particular, the method proposed by~\cite{Kim2016} stands out as it simultaneously estimates the motion of the event camera, constructs a 3D map of the scene, and recovers the intensity image using three parallel filters, which work in tandem to generate an accurate and comprehensive understanding of the scene. Central to the success of this method is incorporating an additional quantity, namely the intensity image, that allows for solving data association by leveraging the Lambertian hypothesis. The approach presented in~\cite{Rebecq2018}, EMVS, involves a space-sweep algorithm that back-projects events into space, creating a ray density volume. Hence, the method can estimate the depth by identifying the density's local maxima. Critically, this approach does not require the recovery of intensity images nor the establishment of event matches, making it highly computationally efficient. However, the demonstration of the EMVS method assumes a known camera trajectory.


==> sections/6-object_motion.old.tex <==
\subsection{Moving Object Detection}
Motion detection is one application that exemplifies the advantages of the neuromorphic photoreceptor compared to standard cameras. 
Due to the design of its photoreceptor and output data structure, this sensor can deliver higher accuracy and faster temporal reaction than the standard camera. 
Detecting moving objects has been extensively studied in computer vision, with various approaches and techniques developed over the years. Traditional cameras are widely used for these applications as the intensity image frames help recognize objects and actions but cannot directly measure motion. Unlike conventional static cameras, which capture images at a fixed rate and resolution, neuromorphic cameras capture only the changes in a scene. The result is a much more efficient and precise method of detecting motion.
Therefore, one of the main advantages of event cameras is that events are solely caused by the motion of objects in the scene, assuming constant illumination. This feature simplifies the segmentation of moving objects when the camera is stationary~\cite{Litzenberger2006a}. However, in scenarios where the camera is moving, events are triggered by both the motion of objects and the camera's ego motion, making it challenging to classify each event's cause. For example,~\cite{Glover2016} test object detection and tracking with an iCub robot trying to catch a ball while moving its head and torso on which the event camera can freely move. These movements cause background clutter, which they can eliminate thanks to the proposed extension of a Hough-based circle detection with optical flow techniques that effectively detect the ball at 500Hz. The approach was later improved through a particle filter that offers a multi-hypothesis on the target state and an adaptive temporal window that can cope with varying speeds and false detections. Alternatively,~\citet{Vasco2017} detect and track more generic object shapes by leveraging additional knowledge of the iCub robot joints controlling the camera motion and using this information to track corners extracted from the event stream. Hence, they first learn a model that correlates joint velocity with the visual motion to separate independently moving objects in a later phase.

Motion segmentation has been addressed by leveraging the idea of motion-compensated event images~\cite{Gallego2018}. Concisely, this technique optimizes the parameter of a warping function so that the events produce sharp edges when projected on a 2D image plane according to a contrast metric. \citet{Mitrokhin2018} detect moving objects in clutter by fitting a motion-compensation model to the dominant events and detecting inconsistencies. \citet{Stoffregen2019} propose an iterative clustering algorithm that jointly estimates the event-object associations and the motion parameters of the objects that produce the sharpest motion-compensated event images. 


Finally, a learning-based approach for segmentation using motion compensation is proposed by~\citet{Mitrokhin2019}. Artificial neural networks estimate depth, ego-motion, segmentation masks of independently moving objects, and object 3D velocities. The authors also release an event-based dataset for supervised learning, which includes accurate pixel-wise motion masks of 3D-scanned objects that are reliable even in poor lighting conditions and during fast motion.

% Building on this foundation, early works focused on refining deep learning techniques for motion segmentation. These models learned to separate ego-motion from independently moving objects directly from event data. The EVIMO dataset, introduced in this period, extended EV-IMO by offering more objects and refined ground-truth motion masks. Methods like Unsupervised Event Segmentation~\cite{Wang2021unsupervised} and event CNNs~\cite{Sekikawa2022eventcnn} explored ways to detect motion without dense supervision, while preserving the advantages of high temporal resolution. These efforts laid the groundwork for later transformer-based and semi-supervised models, showing that event streams alone could support end-to-end learning for motion segmentation.
Building on these motion-compensation-based methods, subsequent research began incorporating deep learning to directly process the spatiotemporal structure of event streams. Early models experimented with convolutional networks and motion-aligned event representations to separate independently moving objects from background motion. During this time,\citet{Mitrokhin2020evimo} introduced the EVIMO dataset, which extended EV-IMO with multiple moving objects, high-quality depth, and motion labels, enabling supervised learning for segmentation tasks. Meanwhile,\citet{Sekikawa2022eventcnn} proposed efficient event CNNs using time surfaces for object-centric motion segmentation. These works formed the basis for more scalable and general models that would emerge in later years.

% Starting in 2023, research in event-based object detection and segmentation advanced rapidly. With the rise of deep learning, new models were designed specifically for the sparse and asynchronous nature of event data. These methods go beyond motion compensation and leverage learned representations to handle complex scenes.

% One notable example is the Recurrent Vision Transformer (RVT) by~\citet{Gehrig2023rvt}. It introduces a transformer-based architecture for object detection that processes spatiotemporal features from events in real-time. The model uses local and global attention mechanisms and recurrent temporal aggregation. It achieves state-of-the-art accuracy on automotive benchmarks such as the Prophesee GEN1 dataset while maintaining low latency of under 12 milliseconds.

% In dynamic environments with ego-motion, moving object segmentation becomes more challenging. To address this,~\citet{Zhou2024emoformer} proposed EmoFormer, a transformer-based model that uses events only during training. Events act as motion priors to supervise a segmentation network, which later runs on standard images alone. This allows accurate motion segmentation without using event data at inference time. Their DSEC-MOS dataset provides pixel-wise annotations for urban driving scenes, filling a critical gap in supervised training data.

% Similarly,~\citet{Georgoulis2024outofroom} introduced a method that first compensates for ego-motion using monocular depth and pose estimates. Then, it segments moving objects in the residual motion of the event stream. This two-stage pipeline improves segmentation quality in outdoor scenarios and sets new benchmarks on EV-IMO and DSEC-MOTS datasets.

% To reduce dependency on labeled data, unsupervised and label-efficient methods have emerged. \citet{Wang2023unev} presented Un-EvMoSeg, an unsupervised approach that detects independently moving objects using geometric inconsistencies in the event flow. Without any manual labels, it achieves competitive results on standard benchmarks. In parallel,~\citet{Wu2024leod} developed LEOD, a semi-supervised framework that trains object detectors using a small portion of labeled events. The model refines pseudo-labels using temporal consistency and achieves strong performance with minimal supervision.

% Apart from learning-based methods, bio-inspired and model-free techniques have also gained attention. \citet{Bak2024oms} proposed a retina-inspired motion segmentation algorithm based on Object Motion Sensitivity (OMS). It mimics the biological retina to suppress ego-motion and isolate independent object motion using simple spatial-temporal filtering. This method requires no training and runs efficiently.

% Another non-learning approach is JSTR by~\citet{Zhou2024jstr}. It combines IMU-based ego-motion compensation with geometric reasoning in the event stream. Events are first aligned using inertial data, and moving objects are detected by clustering inconsistent motion patterns over time. This joint spatio-temporal method achieves robust segmentation without deep networks.

% Finally, hybrid models that fuse events with other modalities have shown promising results. For instance,~\citet{Zhou2023renet} introduced RENet, a dual-stream network that combines events and RGB images for moving object detection. It uses multi-scale temporal aggregation and bi-directional attention to align motion cues from events with semantic features from images. Trained on the DSEC-MOD dataset, RENet performs well across diverse lighting and motion conditions.

% These recent contributions demonstrate the maturity of event-based motion detection. The field has progressed from handcrafted models and small datasets to advanced transformer architectures, unsupervised learning, and large-scale real-world benchmarks. Event-based segmentation now offers not only accuracy and speed but also energy efficiency and robustness, making it suitable for real-time applications in robotics and autonomous systems.
